A Limit Theory of Foundation Models: A Mathematical Approach to Understanding Emergent Intelligence and Scaling Laws

Emergent intelligence have played a major role in the modern AI development. While existing studies primarily rely on empirical observations to characterize this phenomenon, a rigorous theoretical framework remains underexplored. This study attempts to develop a mathematical approach to formalize emergent intelligence from the perspective of limit theory. Specifically, we introduce a performance function E(N, P, K), dependent on data size N, model size P and training steps K, to quantify intelligence behavior. We posit that intelligence emerges as a transition from finite to effectively infinite knowledge, and thus recast emergent intelligence as existence of the limit $\lim_{N,P,K \to \infty} \mathcal{E}(N,P,K)$, with emergent abilities corresponding to the limiting behavior. This limit theory helps reveal that emergent intelligence originates from the existence of a parameter-limit architecture (referred to as the limit architecture), and that emergent intelligence rationally corresponds to the learning behavior of this limit system. By introducing tools from nonlinear Lipschitz operator theory, we prove that the necessary and sufficient conditions for existence of the limit architecture. Furthermore, we derive the scaling law of foundation models by leveraging tools of Lipschitz operator and covering number. Theoretical results show that: 1) emergent intelligence is governed by three key factors-training steps, data size and the model architecture, where the properties of basic blocks play a crucial role in constructing foundation models; 2) the critical condition Lip(T)=1 for emergent intelligence provides theoretical support for existing findings. 3) emergent intelligence is determined by an infinite-dimensional system, yet can be effectively realized in practice through a finite-dimensional architecture. Our empirical results corroborate these theoretical findings.

==> v4/figures.tex <==
% Auto-generated figure gallery. Do not edit manually.
%\section{Comprehensive Visualization}

% Auto-generated figure gallery. Do not edit manually.
%\section{Comprehensive Visualization}
%For each model architecture, we provide two dedicated figures: one for Euclidean distance and one for Cosine similarity. In each figure, rows correspond to task groups (QA, Math, Summ, MT) and columns correspond to the selected layer indices $k$ available in the current result set.

\newcommand{\figurematrixsetup}{%
	\setlength{\tabcolsep}{2pt}%
	\renewcommand{\arraystretch}{1.08}%
	\small%
}

\newcommand{\resultimg}[5]{%
	\begingroup
	\edef\resolvedimagepath{#1/#2#3_#4_input_#5.pdf}%
	\edef\resolvedimage{%
		\noexpand\endgroup
		\noexpand\includegraphics[width=\noexpand\linewidth]{\resolvedimagepath}%
	}%
	\resolvedimage
}

\newcommand{\layerheaderfive}[5]{%
	\textbf{Task} & \textbf{$k=#1$} & \textbf{$k=#2$} & \textbf{$k=#3$} & \textbf{$k=#4$} & \textbf{$k=#5$} \\
}

\newcommand{\taskrowfive}[7]{%
	\textbf{#1} &
	\resultimg{\modeldir}{\modelprefix}{#2}{#3}{\metrictag} &
	\resultimg{\modeldir}{\modelprefix}{#2}{#4}{\metrictag} &
	\resultimg{\modeldir}{\modelprefix}{#2}{#5}{\metrictag} &
	\resultimg{\modeldir}{\modelprefix}{#2}{#6}{\metrictag} &
	\resultimg{\modeldir}{\modelprefix}{#2}{#7}{\metrictag} \\
}

\begin{figure}[p]
	\centering
	\def\modeldir{meta-llama_Llama-3.1-8B}
	\def\modelprefix{datasets_}
	\def\metrictag{eu}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{1}{6}{12}{19}{25}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{1}{6}{12}{19}{25}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{1}{6}{12}{19}{25}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{1}{6}{12}{19}{25}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{1}{6}{12}{19}{25}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of Euclidean distance across each layers for Llama-3.1-8.}
	\label{fig:llama31-8b-eu}
\end{figure}

\begin{figure}[p]
	\centering
	\def\modeldir{meta-llama_Llama-3.1-8B}
	\def\modelprefix{datasets_}
	\def\metrictag{cos}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{1}{6}{12}{19}{25}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{1}{6}{12}{19}{25}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{1}{6}{12}{19}{25}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{1}{6}{12}{19}{25}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{1}{6}{12}{19}{25}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of cosine similarity across each layers for Llama-3.1-8B.}
	\label{fig:llama31-8b-cos}
\end{figure}
\clearpage

\begin{figure}[p]
	\centering
	\def\modeldir{meta-llama_Llama-3.1-70B}
	\def\modelprefix{datasets_}
	\def\metrictag{eu}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{4}{16}{32}{48}{64}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{4}{16}{32}{48}{64}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of Euclidean distance across each layers for Llama-3.1-70B.}
	%	Visualization matrix for Llama-3.1-70B (Dense) using Euclidean Distance. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to the selected layer indices $k \in \{4, 16, 32, 48, 64\}$. This figure emphasizes magnitude changes in representation space.}
	\label{fig:llama31-70b-eu}
\end{figure}

\begin{figure}[p]
	\centering
	\def\modeldir{meta-llama_Llama-3.1-70B}
	\def\modelprefix{datasets_}
	\def\metrictag{cos}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{4}{16}{32}{48}{64}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{4}{16}{32}{48}{64}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of Cosine similarity across each layers for Llama-3.1-70B.}
		%Visualization matrix for Llama-3.1-70B (Dense) using Cosine Similarity. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to the selected layer indices $k \in \{4, 16, 32, 48, 64\}$. This figure emphasizes directional similarity in representation space.}
	\label{fig:llama31-70b-cos}
\end{figure}
\clearpage

\begin{figure}[p]
	\centering
	\def\modeldir{Qwen_Qwen2-7B}
	\def\modelprefix{datasets_}
	\def\metrictag{eu}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{1}{5}{11}{16}{22}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{1}{5}{11}{16}{22}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of Euclidean distance across each layers for Qwen-2-7B.}
		%Visualization matrix for Qwen-2-7B (Dense) using Euclidean Distance. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to the selected layer indices $k \in \{1, 5, 11, 16, 22\}$. This figure emphasizes magnitude changes in representation space.}
	\label{fig:qwen2-7b-eu}
\end{figure}

\begin{figure}[p]
	\centering
	\def\modeldir{Qwen_Qwen2-7B}
	\def\modelprefix{datasets_}
	\def\metrictag{cos}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{1}{5}{11}{16}{22}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{1}{5}{11}{16}{22}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of cosine similarity across each layers for Qwen-2-7B.}
		%Visualization matrix for Qwen-2-7B (Dense) using Cosine Similarity. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to the selected layer indices $k \in \{1, 5, 11, 16, 22\}$. This figure emphasizes directional similarity in representation space.}
	\label{fig:qwen2-7b-cos}
\end{figure}
\clearpage

\begin{figure}[p]
	\centering
	\def\modeldir{Qwen_Qwen2-72B}
	\def\modelprefix{datasets_}
	\def\metrictag{eu}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{4}{16}{32}{48}{64}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{4}{16}{32}{48}{64}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of Euclidean distance across each layers for Qwen-2-72B.}
		%isualization matrix for Qwen-2-72B (Dense) using Euclidean Distance. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to the selected layer indices $k \in \{4, 16, 32, 48, 64\}$. This figure emphasizes magnitude changes in representation space.}
	\label{fig:qwen2-72b-eu}
\end{figure}

\begin{figure}[p]
	\centering
	\def\modeldir{Qwen_Qwen2-72B}
	\def\modelprefix{datasets_}
	\def\metrictag{cos}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{4}{16}{32}{48}{64}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{4}{16}{32}{48}{64}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{4}{16}{32}{48}{64}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of cosine similarity across each layers for Qwen-2-72B.}
	%{Visualization matrix for Qwen-2-72B (Dense) using Cosine Similarity. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to the selected layer indices $k \in \{4, 16, 32, 48, 64\}$. This figure emphasizes directional similarity in representation space.}
	\label{fig:qwen2-72b-cos}
\end{figure}
\clearpage

\begin{figure}[p]
	\centering
	\def\modeldir{deepseek-ai_deepseek-moe-16b-base}
	\def\modelprefix{datasets_}
	\def\metrictag{eu}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{1}{5}{11}{16}{22}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{1}{5}{11}{16}{22}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of Euclidean distance across each layers for Deepseek-MoE-16B.}
	%	Visualization matrix for Deepseek-MoE-16B (MoE) using Euclidean Distance. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to the selected layer indices $k \in \{1, 5, 11, 16, 22\}$. This figure emphasizes magnitude changes in representation space.}
	\label{fig:deepseek-moe-16b-eu}
\end{figure}

\begin{figure}[p]
	\centering
	\def\modeldir{deepseek-ai_deepseek-moe-16b-base}
	\def\modelprefix{datasets_}
	\def\metrictag{cos}
	\figurematrixsetup
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{5}{>{\centering\arraybackslash}m{0.172\textwidth}}}
			\toprule
			\layerheaderfive{1}{5}{11}{16}{22}
			\midrule
			\taskrowfive{QA}{rajpurkar_squad}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{Math}{openai_gsm8k}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{Summ}{knkarthick_dialogsum}{1}{5}{11}{16}{22}
			\addlinespace[2pt]
			\taskrowfive{MT}{Fannyjrd_fair_translate_fr}{1}{5}{11}{16}{22}
			\bottomrule
		\end{tabular}%
	}
	\caption{Visualization of cosine similarity across each layers for Deepseek-MoE-16B.}
	%{Visualization matrix for Deepseek-MoE-16B (MoE) using Cosine Similarity. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to the selected layer indices $k \in \{1, 5, 11, 16, 22\}$. This figure emphasizes directional similarity in representation space.}
	\label{fig:deepseek-moe-16b-cos}
\end{figure}
\clearpage





%\begin{figure}[p] \vspace{-4mm}
%\centering
%\setlength{\tabcolsep}{0.5pt}
%\renewcommand{\arraystretch}{0.9}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=1$} & \textbf{$k=3$} & \textbf{$k=16$} & \textbf{$k=28$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_rajpurkar___squad_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_rajpurkar___squad_3_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_rajpurkar___squad_16_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_rajpurkar___squad_28_input_eu.pdf}} \\
%\addlinespace[0.5pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_openai___gsm8k_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_openai___gsm8k_3_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_openai___gsm8k_16_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_openai___gsm8k_28_input_eu.pdf}} \\
%\addlinespace[0.5pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_knkarthick___dialogsum_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_knkarthick___dialogsum_3_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_knkarthick___dialogsum_16_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_knkarthick___dialogsum_28_input_eu.pdf}} \\
%\addlinespace[0.5pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_Fannyjrd___fair_translate_fr_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_Fannyjrd___fair_translate_fr_3_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_Fannyjrd___fair_translate_fr_16_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_Fannyjrd___fair_translate_fr_28_input_eu.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of Euclidean distance across each layers for Llama-3.1-8. }  \vspace{-4mm}
%\label{fig:llama31-8b-eu}
%\end{figure}
%
%\begin{figure}[htbp]  \vspace{-4mm}
%\centering
%\setlength{\tabcolsep}{0.5pt}
%\renewcommand{\arraystretch}{0.9}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=1$} & \textbf{$k=3$} & \textbf{$k=16$} & \textbf{$k=28$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_rajpurkar___squad_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_rajpurkar___squad_3_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_rajpurkar___squad_16_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_rajpurkar___squad_28_input_cos.pdf}} \\
%\addlinespace[0.5pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_openai___gsm8k_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_openai___gsm8k_3_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_openai___gsm8k_16_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_openai___gsm8k_28_input_cos.pdf}} \\
%\addlinespace[0.5pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_knkarthick___dialogsum_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_knkarthick___dialogsum_3_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_knkarthick___dialogsum_16_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_knkarthick___dialogsum_28_input_cos.pdf}} \\
%\addlinespace[0.5pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_Fannyjrd___fair_translate_fr_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_Fannyjrd___fair_translate_fr_3_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_Fannyjrd___fair_translate_fr_16_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-8B/._datasets_Fannyjrd___fair_translate_fr_28_input_cos.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of cosine distance across each layers for Llama-3.1-8B. } \vspace{-4mm}
%\label{fig:llama31-8b-cos}
%\end{figure}
%
%
%\begin{figure}[p]
%\centering
%\setlength{\tabcolsep}{0.5pt}
%\renewcommand{\arraystretch}{0.9}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=4$} & \textbf{$k=8$} & \textbf{$k=40$} & \textbf{$k=72$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_rajpurkar___squad_4_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_rajpurkar___squad_8_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_rajpurkar___squad_40_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_rajpurkar___squad_72_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_openai___gsm8k_4_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_openai___gsm8k_8_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_openai___gsm8k_40_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_openai___gsm8k_72_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_knkarthick___dialogsum_4_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_knkarthick___dialogsum_8_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_knkarthick___dialogsum_40_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_knkarthick___dialogsum_72_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_Fannyjrd___fair_translate_fr_4_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_Fannyjrd___fair_translate_fr_8_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_Fannyjrd___fair_translate_fr_40_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_Fannyjrd___fair_translate_fr_72_input_eu.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of Euclidean distance across each layers for Llama-3.1-70B.
%	%Visualization matrix for Llama-3.1-70B (Dense) using Euclidean Distance. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to selected layer indices $k \in \{4, 8, 40, 72\}$. This figure emphasizes magnitude changes in representation space.
%	} \vspace{-4mm}
%\label{fig:llama31-70b-eu}
%\end{figure}
%
%\begin{figure}[p]
%\centering
%\setlength{\tabcolsep}{0.5pt}
%\renewcommand{\arraystretch}{0.9}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=4$} & \textbf{$k=8$} & \textbf{$k=40$} & \textbf{$k=72$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_rajpurkar___squad_4_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_rajpurkar___squad_8_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_rajpurkar___squad_40_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_rajpurkar___squad_72_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_openai___gsm8k_4_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_openai___gsm8k_8_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_openai___gsm8k_40_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_openai___gsm8k_72_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_knkarthick___dialogsum_4_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_knkarthick___dialogsum_8_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_knkarthick___dialogsum_40_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_knkarthick___dialogsum_72_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_Fannyjrd___fair_translate_fr_4_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_Fannyjrd___fair_translate_fr_8_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_Fannyjrd___fair_translate_fr_40_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/meta-llama_Llama-3.1-70B/._datasets_Fannyjrd___fair_translate_fr_72_input_cos.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of cosine distance across each layers for Llama-3.1-70B.
%	%Visualization matrix for Llama-3.1-70B (Dense) using Cosine Similarity. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to selected layer indices $k \in \{4, 8, 40, 72\}$. This figure emphasizes directional similarity in representation space.
%	}
%\label{fig:llama31-70b-cos}
%\end{figure}
%\clearpage
%
%\begin{figure}[p]
%\centering
%\setlength{\tabcolsep}{0.5pt}
%\renewcommand{\arraystretch}{0.9}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=1$} & \textbf{$k=2$} & \textbf{$k=14$} & \textbf{$k=25$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_rajpurkar___squad_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_rajpurkar___squad_2_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_rajpurkar___squad_14_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_rajpurkar___squad_25_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_openai___gsm8k_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_openai___gsm8k_2_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_openai___gsm8k_14_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_openai___gsm8k_25_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_knkarthick___dialogsum_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_knkarthick___dialogsum_2_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_knkarthick___dialogsum_14_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_knkarthick___dialogsum_25_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_Fannyjrd___fair_translate_fr_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_Fannyjrd___fair_translate_fr_2_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_Fannyjrd___fair_translate_fr_14_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_Fannyjrd___fair_translate_fr_25_input_eu.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of Euclidean distance across each layers for Qwen-2-7B.
%	%Visualization matrix for Qwen-2-7B (Dense) using Euclidean Distance. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to selected layer indices $k \in \{1, 2, 14, 25\}$. This figure emphasizes magnitude changes in representation space.
%	}
%\label{fig:qwen2-7b-eu}
%\end{figure}
%
%\begin{figure}[p]
%\centering
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{1.05}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=1$} & \textbf{$k=2$} & \textbf{$k=14$} & \textbf{$k=25$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_rajpurkar___squad_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_rajpurkar___squad_2_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_rajpurkar___squad_14_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_rajpurkar___squad_25_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_openai___gsm8k_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_openai___gsm8k_2_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_openai___gsm8k_14_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_openai___gsm8k_25_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_knkarthick___dialogsum_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_knkarthick___dialogsum_2_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_knkarthick___dialogsum_14_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_knkarthick___dialogsum_25_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_Fannyjrd___fair_translate_fr_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_Fannyjrd___fair_translate_fr_2_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_Fannyjrd___fair_translate_fr_14_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-7B/__datasets_Fannyjrd___fair_translate_fr_25_input_cos.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of cosine distance across each layers for Qwen-2-7B.
%	%Visualization matrix for Qwen-2-7B (Dense) using Cosine Similarity. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to selected layer indices $k \in \{1, 2, 14, 25\}$. This figure emphasizes directional similarity in representation space.
%	}
%\label{fig:qwen2-7b-cos}
%\end{figure}
%\clearpage
%
%\begin{figure}[p]
%\centering
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{1.05}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=4$} & \textbf{$k=8$} & \textbf{$k=40$} & \textbf{$k=72$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_rajpurkar___squad_4_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_rajpurkar___squad_8_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_rajpurkar___squad_40_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_rajpurkar___squad_72_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_openai___gsm8k_4_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_openai___gsm8k_8_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_openai___gsm8k_40_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_openai___gsm8k_72_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_knkarthick___dialogsum_4_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_knkarthick___dialogsum_8_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_knkarthick___dialogsum_40_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_knkarthick___dialogsum_72_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_Fannyjrd___fair_translate_fr_4_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_Fannyjrd___fair_translate_fr_8_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_Fannyjrd___fair_translate_fr_40_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_Fannyjrd___fair_translate_fr_72_input_eu.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of Euclidean distance across each layers for Qwen-2-72B.}
%	%Visualization matrix for Qwen-2-72B (Dense) using Euclidean Distance. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to selected layer indices $k \in \{4, 8, 40, 72\}$. This figure emphasizes magnitude changes in representation space.
%\label{fig:qwen2-72b-eu}
%\end{figure}
%
%\begin{figure}[p]
%\centering
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{1.05}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=4$} & \textbf{$k=8$} & \textbf{$k=40$} & \textbf{$k=72$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_rajpurkar___squad_4_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_rajpurkar___squad_8_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_rajpurkar___squad_40_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_rajpurkar___squad_72_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_openai___gsm8k_4_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_openai___gsm8k_8_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_openai___gsm8k_40_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_openai___gsm8k_72_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_knkarthick___dialogsum_4_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_knkarthick___dialogsum_8_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_knkarthick___dialogsum_40_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_knkarthick___dialogsum_72_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_Fannyjrd___fair_translate_fr_4_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_Fannyjrd___fair_translate_fr_8_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_Fannyjrd___fair_translate_fr_40_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/Qwen_Qwen2-72B/__datasets_Fannyjrd___fair_translate_fr_72_input_cos.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of cosine distance across each layers for Qwen-2-72B.
%%	Visualization matrix for Qwen-2-72B (Dense) using Cosine Similarity. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to selected layer indices $k \in \{4, 8, 40, 72\}$. This figure emphasizes directional similarity in representation space.
%	}
%\label{fig:qwen2-72b-cos}
%\end{figure}
%\clearpage
%
%\begin{figure}[p]
%\centering
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{1.05}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=1$} & \textbf{$k=2$} & \textbf{$k=14$} & \textbf{$k=25$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_rajpurkar___squad_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_rajpurkar___squad_2_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_rajpurkar___squad_14_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_rajpurkar___squad_25_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_openai___gsm8k_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_openai___gsm8k_2_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_openai___gsm8k_14_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_openai___gsm8k_25_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_knkarthick___dialogsum_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_knkarthick___dialogsum_2_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_knkarthick___dialogsum_14_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_knkarthick___dialogsum_25_input_eu.pdf}} \\
%\addlinespace[1pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_Fannyjrd___fair_translate_fr_1_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_Fannyjrd___fair_translate_fr_2_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_Fannyjrd___fair_translate_fr_14_input_eu.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_Fannyjrd___fair_translate_fr_25_input_eu.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of Euclidean distance across each layers for Deepseek-MoE-16B.
%	%Visualization matrix for Deepseek-MoE-16B (MoE) using Euclidean Distance. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to selected layer indices $k \in \{1, 2, 14, 25\}$. This figure emphasizes magnitude changes in representation space.
%	}
%\label{fig:deepseek-moe-16b-eu}
%\end{figure}
%
%\begin{figure}[p]
%\centering
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{1.05}
%\small
%\begin{tabular}{>{\centering\arraybackslash}m{0.09\textwidth}*{4}{>{\centering\arraybackslash}m{0.215\textwidth}}}
%\toprule
%\textbf{Task} & \textbf{$k=1$} & \textbf{$k=2$} & \textbf{$k=14$} & \textbf{$k=25$} \\
%\midrule
%\textbf{QA} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_rajpurkar___squad_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_rajpurkar___squad_2_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_rajpurkar___squad_14_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_rajpurkar___squad_25_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{Math} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_openai___gsm8k_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_openai___gsm8k_2_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_openai___gsm8k_14_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_openai___gsm8k_25_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{Summ} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_knkarthick___dialogsum_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_knkarthick___dialogsum_2_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_knkarthick___dialogsum_14_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_knkarthick___dialogsum_25_input_cos.pdf}} \\
%\addlinespace[1pt]
%\textbf{MT} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_Fannyjrd___fair_translate_fr_1_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_Fannyjrd___fair_translate_fr_2_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_Fannyjrd___fair_translate_fr_14_input_cos.pdf}} & \includegraphics[width=0.8\linewidth]{\detokenize{result/deepseek-ai_deepseek-moe-16b-base/._datasets_Fannyjrd___fair_translate_fr_25_input_cos.pdf}} \\
%\bottomrule
%\end{tabular}
%\caption{Visualization of cosine distance across each layers for Deepseek-MoE-16B.
%	%Visualization matrix for Deepseek-MoE-16B (MoE) using Cosine Similarity. Task rows map to datasets as QA=SQuAD, Math=GSM8K, Summ=DialogSum, and MT=fair\_translate\_fr. Columns correspond to selected layer indices $k \in \{1, 2, 14, 25\}$. This figure emphasizes directional similarity in representation space.
%	}
%\label{fig:deepseek-moe-16b-cos}
%\end{figure}
%\clearpage

